Faster Algorithms for Quantitative Verification in Constant Treewidth Graphs

We consider the core algorithmic problems related to verification of systems with respect to three classical quantitative properties, namely, the mean-payoff property, the ratio property, and the minimum initial credit for energy property. The algorithmic problem given a graph and a quantitative property asks to compute the optimal value (the infimum value over all traces) from every node of the graph. We consider graphs with constant treewidth, and it is well-known that the control-flow graphs of most programs have constant treewidth. Let $n$ denote the number of nodes of a graph, $m$ the number of edges (for constant treewidth graphs $m=O(n)$) and $W$ the largest absolute value of the weights. Our main theoretical results are as follows. First, for constant treewidth graphs we present an algorithm that approximates the mean-payoff value within a multiplicative factor of $\epsilon$ in time $O(n \cdot \log (n/\epsilon))$ and linear space, as compared to the classical algorithms that require quadratic time. Second, for the ratio property we present an algorithm that for constant treewidth graphs works in time $O(n \cdot \log (|a\cdot b|))=O(n\cdot\log (n\cdot W))$, when the output is $\frac{a}{b}$, as compared to the previously best known algorithm with running time $O(n^2 \cdot \log (n\cdot W))$. Third, for the minimum initial credit problem we show that (i) for general graphs the problem can be solved in $O(n^2\cdot m)$ time and the associated decision problem can be solved in $O(n\cdot m)$ time, improving the previous known $O(n^3\cdot m\cdot \log (n\cdot W))$ and $O(n^2 \cdot m)$ bounds, respectively; and (ii) for constant treewidth graphs we present an algorithm that requires $O(n\cdot \log n)$ time, improving the previous known $O(n^4 \cdot \log (n \cdot W))$ bound.

==> fig_update.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[thick, >=latex,
pre/.style={<-,shorten >= 1pt, shorten <=1pt, thick},
post/.style={->,shorten >= 1pt, shorten <=1pt,  thick},
und/.style={very thick, draw=gray},
bag/.style={ellipse, minimum height=7mm,minimum width=15mm,draw=black!100, very thick, inner sep=0},
fakebag/.style={ellipse, minimum height=6mm,minimum width=12mm,draw=black!100, very thick},
node/.style={circle, minimum size=2mm, draw=black!100, line width=1pt, inner sep=3},
rootbag/.style={ellipse, minimum height=7mm,minimum width=14mm,draw=black!80, line width=2.5pt},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0},
scale=1,every node/.style={scale=1}]

\def \distdown{0.1cm}
\def \disthor{0.2cm}

\node[bag, ]	at	(0,0) (Bz)	{$z$}; 
\node[fakebag, below = \disthor of  Bz, draw=black!0]	 (H1)	{$\dots$}; 
\node[bag, below  left =\distdown and  \disthor of  H1]	 (B')	{$z,\dots$}; 
\node[fakebag, below  left =\distdown and \disthor of  B', draw=black!0]	 (H2)	{$\dots$}; 
\node[bag, below  left =\distdown and  \disthor of  H2]	 (By)	{ $x,w, z,\dots $}; 
%\node[fakebag, below  right =\distdown and  \disthor of  Bz, draw=black!0]	 (H3)	{$\dots$}; 
\node[fakebag, below  right =\distdown and  \disthor of  B', draw=black!0]	 (H4)	{$\dots$}; 
\node[fakebag, below  left =\distdown and  \disthor of  By, draw=black!0]	 (H5)	{$\dots$}; 
\node[fakebag, below  right =\distdown and  \disthor of  By, draw=black!0]	 (H6)	{$\dots$}; 

\draw [draw=black, thick, shorten >=-2.5mm] (Bz) to (H1);
%\draw [draw=black, thick, shorten >=-2.5mm] (Bz) to (H3);
\draw [draw=black, thick, shorten >=-2.5mm] (B') to (H1);
\draw [draw=black, thick, shorten >=-2.5mm] (B') to (H2);
\draw [draw=black, thick, shorten >=-2.5mm] (By) to (H2);
\draw [draw=black, thick, shorten >=-2.5mm] (B') to (H4);
\draw [draw=black, thick, shorten >=-2.5mm] (By) to (H5);
\draw [draw=black, thick, shorten >=-2.5mm] (By) to (H6);

\node[right = 0.1cm of Bz] {\large $\Bag_z$};
\node[right = 0.1cm of B'] {\large $\Bag'$};
\node[right = 0.1cm of By] {\large $\Bag_y$};

%\draw [draw=black, loop above, looseness=20, line width =1, ->] (x) to node[above=0.2]{$\LD_{\Bag}(x,x)$} (x);

\end{tikzpicture}
\caption{Illustration of path shortening in line~\ref{line:path_shortening} of $\Cyclealgo$.
When $\Bag_x$ is examined, $\LD_{\Bag_x}(u,v)$ is updated with the weight of the $\Ushape$-shaped path $P=P_1\circ P_2$ (i.e., $\Weight(P)=\Weight(P_1) + \Weight(P_2)$).
Here $P_1$ and $P_2$ are $\Ushape$-shaped paths in the children bags of $\Bag_x$, and their weights are stored in $\LD_{\Bag_x}(u,x)$ and $\LD_{\Bag_x}(x,v)$ respectively.}\label{fig:fig_update}
\end{figure}
